Soft dynamics in heavy-light mesons

We compute the radial distributions of the scalar, vector and axial charge density in the heavy-light mesons. We present the results obtained for both the lowest lying static heavy-light mesons as well as for their nearest excitations, with $N_f=2$ dynamical quarks of Wilson (Clover) type. We used various improvements of the static heavy-quark actions. From these distributions we were able to compute the corresponding charges and their radii $< r^2>$, the results of which are also presented.

==> Makefile <==
nirvana:
	latex skeleton.tex
	latex skeleton.tex
	latex skeleton.tex
	dvips -Ppdf -z -G0 skeleton.dvi -o && \
	ps2pdf -sPAPERSIZE=a4 skeleton.ps
	@echo
	@echo
	@echo
	@echo "OUTPUT skeleton.pdf"
	@echo
	@echo
	@echo
clean:
	rm -f *.aux *.dvi *.log *.tmp skeleton.ps *.pdf

